Parallel Approximation of the Maximum Likelihood Estimation for the Prediction of Large-Scale Geostatistics Simulations

Maximum likelihood estimation is an important statistical technique for estimating missing data, for example in climate and environmental applications, which are usually large and feature data points that are irregularly spaced. In particular, the Gaussian log-likelihood function is the \emph{de facto} model, which operates on the resulting sizable dense covariance matrix. The advent of high performance systems with advanced computing power and memory capacity have enabled full simulations only for rather small dimensional climate problems, solved at the machine precision accuracy. The challenge for high dimensional problems lies in the computation requirements of the log-likelihood function, which necessitates ${\mathcal O}(n^2)$ storage and ${\mathcal O}(n^3)$ operations, where $n$ represents the number of given spatial locations. This prohibitive computational cost may be reduced by using approximation techniques that not only enable large-scale simulations otherwise intractable but also maintain the accuracy and the fidelity of the spatial statistics model. In this paper, we extend the Exascale GeoStatistics software framework (i.e., ExaGeoStat) to support the Tile Low-Rank (TLR) approximation technique, which exploits the data sparsity of the dense covariance matrix by compressing the off-diagonal tiles up to a user-defined accuracy threshold. The underlying linear algebra operations may then be carried out on this data compression format, which may ultimately reduce the arithmetic complexity of the maximum likelihood estimation and the corresponding memory footprint. Performance results of TLR-based computations on shared and distributed-memory systems attain up to 13X and 5X speedups, respectively, compared to full accuracy simulations using synthetic and real datasets (up to 2M), while ensuring adequate prediction accuracy.

==> text/abstract.tex <==
\begin{abstract}
\end{abstract}


==> text/lrapprox.tex <==
%!TEX root = ../cluster.tex
\section{Tile Low-Rank Approximation}
\label{sec:TLR}
%\subsection{Independent Blocks Method (IND)}
%
%Reducing the algorithmic complexity is a necessity in the case of very large and irregularly spaced geospatial data. One 
%way is to use a subset of the measurements vector $Z$ to estimate the parameter vector $\widehat{\boldsymbol \theta}$. 
%Several previous studies have proposed different methods, ex., Independent blocks method (IND), Nearest neighbors
%method (NN), Nearest neighboring sets method (SUM), Nearest neighbors and nearest neighboring sets method (NNSUM),
%of this kind of approximation where these methods have shown their effectiveness in both computation and
%accuracy~\cite{datta2016hierarchical, huang2017hierarchical, 2017arXiv170904419L, nychka2015multiresolution, stein2013statistical, sun2016statistically}. 
%
%
%Although, this paper propose a low-rank approximation techniques based on Singular value decomposition (SVD) technique
%, the quality of approximation technique may be demonstrated by comparing it with both exact computation and traditional
%approximation approaches on the same problem. Thus, this section helights one of commonly used approximation
%methods, i.e., Independent blocks method (IND) where only the diagonal tiles are used to estimate the likelihood
%optimized $\widehat{\boldsymbol \theta}$. Such a strategy has been used in different studies and turns out to be a suitable
%way to reduce the complexity of evaluating the likelihood function on large-scale datasets~\cite{huang2017hierarchical, stein2013statistical}. 
%
%
%
%The IND approximation technique proceeds by annihilating off-diagonal tiles, since their contributions 
%as well as their qualitative impact on the overall statistical problem may be limited. 
%
%
%The implementation of this
%approximation technique maps well with the inherent tile algorithms that are used to estimate the MLE function and enables to expose
%tuning parameters, which trades off performance and statistical efficiency.
%
%One of these tunable parameters is the size of the diagonal super tile, which determines how many tiles, around the diagonal,
%need to be aggregated together. A large diagonal super tile basically integrates more statistical contributions from the original problem at the expense of
%performing more operations.
%
%%Figure~\ref{fig:diag-approx} shows an example of the IND approximation technique using a diagonal 2-by-2 super tile matrix.
%
%
%IND approximation technique proceeds by dividing the location matrix into $n/r$ blocks, each of which contains $r$ points.
%Because our framework depends on tile algorithms, each block will contain $n^2$ tiles, where $n={1,..., m/2}$
%and $m$ represents the number of tiles on a single dimension. In this method, several correlations between different
%locations are ignored, i.e., $\bf{\Sigma_{ij}} = 0$. Only diagonal is used for computation and the thick of this diagonal
%depends on the number of tiles per individual diagonal-blocks. 
%
%
%%\begin{figure}
%%	\centering
%%	\includegraphics[width=5 cm, height= 5 cm ]{./figures/diag_approx.pdf}
%%	\caption{An example of Independent Blocks (IND) approximation technique on a diagonal 3-by-3 super tile matrix. }
%%	\label{fig:diag-approx}
%%\end{figure}
%
%The IND approximation technique generates a matrix where elements from off-diagonal 
%tiles are set to zero. In this case, applying Cholesky factorization
%to the whole matrix is unnecessary and time-consuming. Thus, we propose a 
%modified version of the well-known tile Cholesky factorization
%algorithm presented in~\cite{Agullo_2009_jpcs}. The modified version 
%is aware of the new sparse structure of the matrix 
%and avoids zeros-tiles during the computation, which speeds-up the Cholesky 
%factorization operation for the whole matrix.
%
%
%\begin{algorithm} [htp]
%	\setstretch{1}
%	\caption{\bf: Modified Cholesky Algorithm \\(right-looking version)}
%	\label{alg:cholesky}
%	\begin{algorithmic}[1]
%		\State Input:  Positive-definite matrix $\bf{\Sigma}$, number of tiles $tiles$, and number of tiles per subregion $tiles\_subregion$
%		\State Output: The cholesky factorization of $\bf{\Sigma}$:
%		\For{$k = 0 ... tiles-1$ }
%		\State ${\bf \Sigma_{kk}} = dpotrf ({\bf \Sigma_{kk}}  )$ $  \Rightarrow$     Compute the Cholesky factorization.
%				\For {$m = k+1... tiles-1$ and $m < k+diag\_thick$}
%						\State${\bf \Sigma_{kk}} = dtrsm ({\bf \Sigma_{kk}, {\bf \Sigma_{mk}} } )$ $  \Rightarrow$     Compute the solution to a system of linear.
%				\EndFor		
%   				\For {$m = k+1... tiles-1$ and $m < k+diag\_thick$ }
%				       	\For{$n = k+1 ... m$ and $n < m+diag\_thick$}
%				       			      \State  $\bf {\Sigma_{mk}}$= dgemm ($\bf {\Sigma_{kn}}$, $\bf {\Sigma_{mn}}$)   $\Rightarrow$  Performs the matrix-matrix. operation $\bf {Z_{1}= \Sigma_{12} \times X}$
%
%				    	\EndFor
%    	              \State${\bf \Sigma_{kk}} = dsyrk ({\bf \Sigma_{kn}, {\bf \Sigma_{kk}} } )$ $  \Rightarrow$     Compute symmetric rank K-operation.
% 			 \EndFor
%		 \EndFor
%		
%		
%	\end{algorithmic}
%\end{algorithm}

%\subsection{Low Rank (LR) Approximation of Covariance Matrices}

%\subsection{LR Matrices}
%It is well known that processing large sparse matrices is easier than processing a fully dense matrices. 
Covariance
matrices are usually dense with sparsity property.  {\em ExaGeoStat} includes three operations,
i.e., synthetic data generation, MLE , and prediction~\cite{abdulah2017exageostat}. All these
operations depend on generating a large covariance matrices
${\boldsymbol \Sigma}({\boldsymbol \theta})$ - a power-of-two of the
 number of spatial locations - and applying
Cholesky factorization to this covariance matrix. In this case, Cholesky
 factorization is the most time-consuming part, which requires $n^3$ computation
  and $n^2$ memory in the dense case. Both data
generation and prediction operations require one Cholesky factorization which could be acceptable
in dense format if memory is available while the MLE optimization problem involves several calls to the
Cholesky routine which is prohibitive when estimating the maximum likelihood parameter vector
$\widehat{\boldsymbol \theta}$. Thus, speeding-up the Cholesky factorization definitely will
impact the performance of the MLE operation.


Low-Rank (LR) approximation depends on reducing the exact computation complexity by exploiting the
sparsity property of the likelihood covariance matrix. When neighbors  in  a certain region are strongly
correlated, the measurements variation can be represented by low-frequency component ~\cite{stein2014limitations}. In this case, the low-rank approximation could be a suitable approach to reduce the complexity.


Tile-based algorithms have been used recently on manycore architectures
to speed-up parallel linear solvers algorithms~\cite{akbudak-isc17}. Compared to block-based algorithms,
tile-based algorithms  involve multi-threaded BLAS to weaken the synchronizations points in the parallel
algorithms. Thus, 
in this study, we propose a fast MLE optimization framework based on Tile Low-Rank (TLR) variant of
 low-rank approximation which
is faster than dense computation and fulfills the accuracy requirements of the MLE operation.



Our covariance matrix ${\boldsymbol \Sigma}({\boldsymbol \theta})$ is divided into a set of square tiles. Tile size is chosen
based on gained performance (i.e., performance tuned parameter).  Singular Value Decomposition (SVD) or 
is used to approximate each tile alone by representing each tile as
two matrices, significant singular values $U$ and its associated singular vector $V$.  The significance of
each singular value depends on a pre-determined accuracy input which usually an application-specific. The $k$ most significant singular values can be used to represent each single tile as a product of two rectangular matrices $U_{ij}$ and $V_{ij}$ with size $nb \times k$ where $nb$ represents the tile size which is fixed for all matrix tiles and $k$ represents the matrix rank. Thus,
 with higher accuracy threshold, higher $U$ and $V$ ranks are required. The low-rank Cholesky factorization
  depends on approximating all off-diagonal tiles and keeps diagonal tiles as dense.
 
 
We depend on the HiCMA library proposed by our group~\cite{akbudak-isc17} to apply TLR approximation to the MLE problem.
HiCMA provides two LR approximation variants of a given dense matrix: {\em fixed rank} where accuracy is different across
all off-diagonal tiles and a fixed $k$ is used and {\em fixed accuracy} where approximation accuracy is fixed through all
 the off-diagonal tiles and different $k$ values are used for each tile to satisfy the required accuracy. 
 Figure~\ref{fig:lr_representation} shows an example TLR representation of a covariance matrix ${\boldsymbol \Sigma}({\boldsymbol \theta})$. 


 \begin{figure}
\centering
\includegraphics[width=0.5\linewidth]{./figures/fixed_acc.png}
  \caption{TLR representation of a covariance matrix ${\boldsymbol \Sigma}({\boldsymbol \theta})$ with fixed accuracy.}
  \label{fig:lr_representation}
\end{figure}





==> text/numstudy.tex <==
%!TEX root = ../cluster.tex
\section{Numerical Study}

\subsection{Design Setup}
In this study, the synthetic datasets are generated at irregular locations in a two-dimensional space
with an unstructured covariance matrix~\cite{huang2017hierarchical,sun2016statistically}. 
To ensure that no two locations are too close, the data locations are generated using $n^{1/2}(r-0.5+X_{rl},l-0.5+Y_{rl})$ for 
$r,l \in \{1,\dots, n^{1/2}\}$, where $n$ represents the number of locations, and $X_{rl}$ and $Y_{rl}$ 
are generated using uniform distribution on ($-$0.4, 0.4).  
Figure~\ref{fig:irregular-space} shows a drawable example of 400 irregularly spaced grid locations in a square region. We only use such a small example to highlight
our methodology to generate geospatial data, however,  this work uses synthetic datasets up to $49 \times 10^{10}$ locations (i.e., 10 M $\times$ 10 M).

\begin{figure}
	\centering
	\includegraphics[width=4.5 cm, height= 4.5 cm ]{./figures/irregular-space.pdf}
	\caption{An example of  400 points irregularly distributed in space, with 362 points (\textcolor{red}{$\circ$}) for maximum likelihood estimation and 38 points (\textcolor{blue}{$\times$}) for prediction validation.}
	\label{fig:irregular-space}
\end{figure}


In this study, we consider a Zero-mean Gaussian process with Mat\'{e}rn covariance matrix. $10^{-4}$ noise is added to the diagonal elements to keep the matrix positive definite through the maximization process.

\subsection{Dependence level}
Recalling the Mat\'{e}rn covariance kernel in ~\ref{eq:MaternCov}. The range parameter $\theta_2 > 0$ controls the dependence of the process. In this study, we consider three levels of dependences: $\theta_2 = 0.03$ (weak dependency), $\theta_2 = 0.1$ (medium dependency), and $\theta_2 = 0.3 $(strong). To study the impact of different dependency levels using different TLR approximation levels and exact computation, we 
set  the variance $theta_1 = 1$  and the smoothness parameter $theta_3 =0.5$ which represent an exponential covariance function:
 
\begin{equation}
	\label{eq:ExpCov}
	C_{0.5}(r;{\boldsymbol \theta})={\theta_1} exp \frac{-r}{2^{\theta_2}}
\end{equation}


Figure~\ref{fig:dep_comp} shows a set of box-plots with different dependency levels.


\begin{figure*}[!ht]
  \centering
  \subfigure[Estimated variance parameter. ($\theta_1$).]{
    \label{fig:theta1}
   \includegraphics[width=0.32\linewidth, height=0.2\textheight]{./figures/theta1-40k-1-0.1-0.5-mle.pdf}}
  \subfigure[Estimated spatial range parameter. ($\theta_2$).]{
    \label{fig:theta2}
   \includegraphics[width=0.32\linewidth, height=0.2\textheight]{./figures/theta2-40k-1-0.1-0.5-mle.pdf}}
  \subfigure[Estimated smoothness parameter ($\theta_3$).]{
    \label{fig:theta3}
   \includegraphics[width=0.32\linewidth, height=0.2\textheight]{./figures/theta3-40k-1-0.1-0.5-mle.pdf}}
   
     \subfigure[Estimated variance parameter. ($\theta_1$).]{
    \label{fig:theta1}
   \includegraphics[width=0.32\linewidth, height=0.2\textheight]{./figures/theta1-40k-1-0.03-0.5-mle.pdf}}
  \subfigure[Estimated spatial range parameter. ($\theta_2$).]{
    \label{fig:theta2}
   \includegraphics[width=0.32\linewidth, height=0.2\textheight]{./figures/theta2-40k-1-0.03-0.5-mle.pdf}}
  \subfigure[Estimated smoothness parameter ($\theta_3$).]{
    \label{fig:theta3}
   \includegraphics[width=0.32\linewidth, height=0.2\textheight]{./figures/theta3-40k-1-0.03-0.5-mle.pdf}}
   
     \subfigure[Estimated variance parameter. ($\theta_1$).]{
    \label{fig:theta1}
   \includegraphics[width=0.32\linewidth, height=0.2\textheight]{./figures/theta1-40k-1-0.3-0.5-mle.pdf}}
  \subfigure[Estimated spatial range parameter. ($\theta_2$).]{
    \label{fig:theta2}
   \includegraphics[width=0.32\linewidth, height=0.2\textheight]{./figures/theta2-40k-1-0.3-0.5-mle.pdf}}
  \subfigure[Estimated smoothness parameter ($\theta_3$).]{
    \label{fig:theta3}
   \includegraphics[width=0.32\linewidth, height=0.2\textheight]{./figures/theta3-40k-1-0.3-0.5-mle.pdf}}
\caption{Boxplots of parameter estimates ($\theta_1$, $\theta_2$, and $\theta_3$). 
%The solid line is a reference for the true parameter value.
}
\label{fig:dep_comp}
\end{figure*}

\subsection{Smoothness level}
$\theta_3$ in Mat\'{e}rn covariance indicates the smoother process. To study the impact of TLR approximation on different $\theta_3$ values, we fix $theta_1 = 1$ and $theta_2 = 0.1$, i.e., medium dependency. We select two smoothness levels, $theta_3 = 0.5$ and $theta_3 = 1$, which corresponding to the exponential covariance function~\ref{eq:ExpCov} and Whittle covariance function:

\begin{equation}
	\label{eq:ExpCov}
	C_{1}(r;{\boldsymbol \theta})={\theta_1} \frac{r}{\theta_2} {\mathcal K}_{1}(\frac{r}{\theta_2})
\end{equation}


Figure~\ref{fig:smooth_comp} shows a set of box-plots with different dependency levels.


\begin{figure*}[!ht]
  \centering
  \subfigure[Estimated variance parameter. ($\theta_1$).]{
    \label{fig:theta1}
   \includegraphics[width=0.32\linewidth, height=0.2\textheight]{./figures/theta1-40k-1-0.1-1-mle.pdf}}
  \subfigure[Estimated spatial range parameter. ($\theta_2$).]{
    \label{fig:theta2}
   \includegraphics[width=0.32\linewidth, height=0.2\textheight]{./figures/theta2-40k-1-0.1-1-mle.pdf}}
  \subfigure[Estimated smoothness parameter ($\theta_3$).]{
    \label{fig:theta3}
   \includegraphics[width=0.32\linewidth, height=0.2\textheight]{./figures/theta3-40k-1-0.1-1-mle.pdf}}
     \subfigure[Estimated variance parameter. ($\theta_1$).]{
    \label{fig:theta1}
   \includegraphics[width=0.32\linewidth, height=0.2\textheight]{./figures/theta1-40k-1-0.3-1-mle.pdf}}
  \subfigure[Estimated spatial range parameter. ($\theta_2$).]{
    \label{fig:theta2}
   \includegraphics[width=0.32\linewidth, height=0.2\textheight]{./figures/theta2-40k-1-0.3-1-mle.pdf}}
  \subfigure[Estimated smoothness parameter ($\theta_3$).]{
    \label{fig:theta3}
   \includegraphics[width=0.32\linewidth, height=0.2\textheight]{./figures/theta3-40k-1-0.3-1-mle.pdf}}
   \subfigure[Estimated variance parameter. ($\theta_1$).]{
    \label{fig:theta1}
   \includegraphics[width=0.32\linewidth, height=0.2\textheight]{./figures/theta1-40k-1-0.03-1-mle.pdf}}
  \subfigure[Estimated spatial range parameter. ($\theta_2$).]{
    \label{fig:theta2}
   \includegraphics[width=0.32\linewidth, height=0.2\textheight]{./figures/theta2-40k-1-0.03-1-mle.pdf}}
  \subfigure[Estimated smoothness parameter ($\theta_3$).]{
    \label{fig:theta3}
   \includegraphics[width=0.32\linewidth, height=0.2\textheight]{./figures/theta3-40k-1-0.03-1-mle.pdf}}
    
\caption{Boxplots of parameter estimates ($\theta_1$, $\theta_2$, and $\theta_3$). 
%The solid line is a reference for the true parameter value.
}
\label{fig:smooth_comp}
\end{figure*}

==> text/trash/lalib.tex <==
\section{Linear Algebra Libraries}
\label{sec:lalib}
This section recalls the latest developments in both sense and approximate linear
algebra software libraries and their relevant implications.

\subsection{Dense Linear Algebra Library} 
Dense linear solvers have been provided through block or tile algorithms.
LAPACK~\cite{anderson1999lapack} and  ScaLAPACK~\cite{scalapack} 
are a best block-based linear algebra library. 
Figure~\ref{fig:format-cdl} shows the major data layout format in the block algorithms.

LAPACK is well-established open-source dense linear algebra library
for shared-memory systems, is block-column algorithms. 
Block algorithms decompose the matrix into successive panel and
update computational phases, while the matrix is organized in a column-major format.



The matrix transformations are blocked within the 
panel factorization phase, and applied together at one time during
the update phase. The former is typically memory-bound 
due to the Level-2 BLAS operations, while the latter is compute-intensive
due to the Level-3 BLAS updates occurring on the trailing submatrix. LAPACK 
uses the fork-join paradigm, which has demonstrated scalability issues on multicore
architectures. Its distributed version, ScaLAPACK follows the same 
paradigm and scatters the matrix
using a two-dimensional block-cyclic data distribution across a grid of processors
to reduce load imbalance and communication overheads.

\begin{figure}
	\centering

		\subfigure[LAPACK: Column-major data layout format.]{
			\label{fig:format-cdl}
		\includegraphics[width=0.18\textwidth]{./figures/format-cdl}}
		\hspace{5mm}
		\subfigure[Chameleon: Tile data layout format.]{
			\label{fig:format-tdl}
		\includegraphics[width=0.18\textwidth]{./figures/format-tdl}}
	\caption{Data layout format.}
	\label{fig:block-tile-dag}
\end{figure}




Further, the tile algorithm methodology~\cite{Agullo_2009_jpcs,chameleon-soft} 
splits the matrix into small tiles instead of tall panels, as
seen in Figure~\ref{fig:format-tdl},
so that updates of the trailing submatrix may be triggered before the current
panel factorization is complete. This fine-grained lookahead method 
exploits more concurrency and enables the maximization of hardware resources by removing
synchronization points between the panel and update computational
phases. The numerical algorithm can then be translated into a Directed
Acyclic Graph (DAG), where the nodes represent tasks and the edges define data dependencies,
as highlighted in Figure~\ref{fig:dag}.


The 
dense linear algebra library Chameleon~\cite{chameleon-soft} provided a tile-based linear solvers, which breaks down the tasks of the
traditional bulk-synchronous programming model of LAPACK~\cite{anderson1999lapack} and renders them
for an asynchronous task-based programming model. 


\subsection{Approximation Linear Algebra Library} 




\subsection{Dynamic Runtime Systems}

Once the tasks are defined with their respective data
dependencies, a dynamic runtime system~\cite{augonnet2011starpu,duran2009proposal, EdwardsTS14} 
may be employed directly on the sequential code to schedule the
various tasks across the underlying hardware resources. Its role
is to ensure that the data dependencies are not violated. These runtimes enhance the software productivity by abstracting
the hardware complexity from the end users. They are also capable of reducing
load imbalance, mitigating data movement overhead, and increasing occupancy
on the hardware.
